Geometrical tests of cosmological models. I. Probing dark energy using the kinematics of high-redshift galaxies

We suggest to use the observationally measured and theoretically justified correlation between size and rotational velocity of galactic discs as a viable method to select a set of high redshift standard rods which may be used to explore the dark energy content of the universe via the classical angular-diameter test. Here we explore a new strategy for an optimal implementation of this test. We propose to use the rotation speed of high redshift galaxies as a standard size indicator and show how high resolution multi-object spectroscopy and ACS/HST high quality spatial images, may be combined to measure the amplitude of the dark energy density parameter, or to constrain the cosmic equation of state parameter for a smooth dark energy component. We evaluate how systematics may affect the proposed tests, and find that a linear standard rod evolution, causing galaxy dimensions to be up to 30% smaller at z=1.5, can be uniquely diagnosed, and will minimally bias the confidence level contours in the [Omega_Q, w] plane. Finally, we show how to derive, without a priori knowing the specific functional form of disc evolution, a cosmology-evolution diagram with which it is possible to establish a mapping between different cosmological models and the amount of galaxy disc/luminosity evolution expected at a given redshift.

==> macros.tex <==
\def\etal{{et al.~}}
\def\cf{{cf.~}}
\def\eg{{e.g.,~}}
\def\ie{{i.e.,~}}
\def\lsim{\raise0.3ex\hbox{$<$}\kern-0.75em{\lower0.65ex\hbox{$\sim$}}} 
\def\gsim{\raise0.3ex\hbox{$>$}\kern-0.75em{\lower0.65ex\hbox{$\sim$}}} 
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\def\sc1{\raise2.1ex\hbox{\tiny $r\!\!=\!\!4$}\kern-0.95em{\hbox{$=$}}} 

\def\kmsmpc{~{$\rm km~s^{-1}~Mpc^{-1}$}}
\def\Msun{~{\rm M}_{\sun}}
\def\Lsun{~{\rm L}_{\sun}}
\newcommand{\ls}{L\sbr{s}}


\newcommand{\mamo}[1]{\mbox{$#1$}}
\newcommand{\unit}[1]{\ifmmode \:\mbox{\rm #1}\else \mbox{#1}\fi}
\newcommand{\sbr}[1]{_{\rm #1}}

\newcommand{\mone}{\mamo{^{-1}}}            %^{-1}
\newcommand{\km}{\unit{km}}
\newcommand{\kms}{\unit{km~s\mone}}
\newcommand{\kpc}{\unit{kpc}}
\newcommand{\mpc}{\unit{Mpc}}
\newcommand{\hkpc}{\mamo{h\mone}\kpc}       %h^-1 Kpc
\newcommand{\hmpc}{\mamo{h{\mone}\mpc }}     %h^-1 Mpc
\newcommand{\hinvmpcub}{\mamo{h^{-3} \mpc^{3}}}    %h^-3 Mpc^3
\newcommand{\hmpcinvcub}{\mamo{h^{3} \mpc^{-3}}}   %h^3 Mpc^-3
\newcommand{\ten}[1]{\mamo{\times 10^{#1}}}        % .10^

% My def.
\def\hinv{$h^{-1}$}
\def\lcdm{$\Lambda$CDM~}
\def\tcdm{$\tau$CDM~}
%
\def\ltsima{$\; \buildrel < \over \sim \;$}
\def\simlt{\lower.5ex\hbox{\ltsima}}
\def\gtsima{$\; \buildrel > \over \sim \;$}
\def\simgt{\lower.5ex\hbox{\gtsima}}          
%
%               

\def\aapl{{\rm Astr.~Astrophys.~Lett.\ }}
\def\aaps{{\rm Astr.~Astrophys.~Suppl.\ }}
\def\AN{{\rm Astron.~Nachr.\ }}
\def\app{{\rm Astropart.~Phys.\ }}
\def\capss{{\rm Comm.~Astrophys.~Space Sci.\ }}
\def\asr{{\rm Adv.~Space Res.\ }}
\def\az{{\rm Astron.~Zh.\ }}
\def\ic{{\rm Icarus\ }}
\def\mnrasl{{\rm Mon.~Not.~R.~Astron.~Soc.~Lett.\ }}
\def\phd{{\rm PhD thesis\ }}
\def\ps{\physscr}
\def\prp{\physrep}
\def\ppl{{\rm Phys.~Plasma.\ }}
\def\rmp{{\rm Rev.~Mod.~Phys.\ }}
\def\sc{{\rm Science\ }}
\def\ssr{{\rm Space Sci.~Rev.\ }}
\def\rmp{{\rm Rev.\ Mod.\ Phys.\ }}
\def\npb{{\rm Nucl. Phys.\ B }}
\def\jcp{{\rm J.\ Comp.\ Phys.\ }}
\def\cpc{{\rm Comp.\ Phys.\ Comm.\ }}
\def\jgr{{\rm J.\ Geoph.\ Res.\ }}
\def\sovast{\rm{Soviet~Ast.}}
%

